Learning via Self-Consistency for Diffusion-based Video Reasoning

While video diffusion models have demonstrated emerging zero-shot capability for visual reasoning and perception tasks, their stochastic generations often produce inconsistent predictions for tasks requiring reliable, structured outputs. Prior work has shown that self-consistency across stochastic video generations can improve diffusion-based reasoning at test time. We systematically extend the test-time method to structured prediction problems such as referring segmentation. However, test time scaling via self-consistency requires multiple rollouts and incurs much more latency. We propose self-consistency as an intrinsic learning signal for post-training video diffusion models without ground truth annotations or external verifiers. Specifically, our proposed Self-Consistency Fine-Tuning (SC-FT) distills consensus predictions into the video generation model, while subsequent Self-Consistency Reinforcement Learning (SC-RL) rewards generations according to their agreement with the consensus. The resulting model effectively internalizes the benefit of multi-sample consensus and requires only a single generation at inference time, while substantially outperforming the original model. To further reduce inference overhead, we read out predictions early in the denoising trajectory, preserving consensus quality while cutting inference time per rollout by 52%. For visual search, our method raises task accuracy from 48.4% for a single generation to 99.1%. For maze solving across three layout sizes, SC-FT and SC-RL improve single generation strict validity from 59.1% to 66.1% and 95.6% with the same inference latency. Also, for referring segmentation, SC-RL raises single-generation gIoU from 0.402 to 0.582, beyond SC-FT 0.473.

==> preamble.tex <==
%% Fix CVPR review line numbers on TeX Live 2025-06+ (lineno v5.7 writes the column
%% marker one column late, so left/right line numbers land in the gutter).
\makeatletter
\@ifpackageloaded{lineno}{%
  \IfFormatAtLeastTF{2025-06-01}{%
    \RemoveFromHook{build/column/before}[lineno]%
    \AtBeginDocument{%
      \def\@LN@makecol{%
        \@LN@orig@makecol
        \setbox\@outputbox\vbox{%
          \boxmaxdepth\@maxdepth
          \protected@write\@auxout{}{%
            \string\def\string\@LN@column{\if@firstcolumn1\else2\fi}}%
          \box\@outputbox}}%
    }%
  }{}%
}{}
\makeatother

%% Lets \caption work outside a float (teaser under the title, see sections/teaser.tex).
\makeatletter\newcommand{\captionsetuptype}{\def\@captype{figure}}\makeatother

%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}
% \usepackage{etoc}
%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
\setlength{\abovecaptionskip}{3pt}
%%
%% space between floats and text (LaTeX default: 20pt around a float, 12pt between floats, 10pt above a caption).
%% Page size, margins, columns and font sizes of the CVPR style are untouched.
%%
\setlength{\textfloatsep}{8pt plus 2pt minus 2pt}
\setlength{\dbltextfloatsep}{8pt plus 2pt minus 2pt}
\setlength{\floatsep}{6pt plus 2pt minus 2pt}
\setlength{\dblfloatsep}{6pt plus 2pt minus 2pt}
\usepackage{booktabs}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{float}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{placeins}
\usepackage{needspace}
\usepackage{enumitem}
\usepackage{tabularx}
\usepackage{xcolor}
%% Revision of the tables for the CVPR resubmission: everything new is purple.
% Revision colour switched off on 2026-11-14 (was RGB 112,48,160); the \rev markup stays in the sources.
\definecolor{revpurple}{RGB}{0,0,0}
\newcommand{\rev}[1]{\begingroup\color{revpurple}#1\endgroup}
% Revision colour switched off on 2026-11-14 (was RGB 230,105,0); the \revorange markup stays in the sources.
\definecolor{revorange}{RGB}{0,0,0}
\newcommand{\revorange}[1]{\begingroup\color{revorange}#1\endgroup}
%% Coauthor edit markers (shared by main.tex and supp.tex).
\newcommand{\rebuttal}[1]{\begingroup\color{black}#1\endgroup}
\newcommand{\meng}[1]{\textcolor{black}{#1}}
%% Paper title, used by both main.tex and supp.tex.
\newcommand{\papertitle}{Learning via Self-Consistency for Diffusion-based Video Reasoning}
%% Shrink a table panel to the available width (never enlarges it).
\newcommand{\fitpanel}[1]{\resizebox{\ifdim\width>\linewidth\linewidth\else\width\fi}{!}{#1}}
\usepackage{microtype}
% etoc (table-of-contents control) was removed on 2026-11-16: no table of contents is printed, and it
% loads multicol, which warns under the twocolumn option.
% \usepackage[colorlinks=true,allcolors=blue]{hyperref}
\urlstyle{same}
%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}
